ToWo-VTON: Take-Off Wear-On Virtual Try-On via Topology-aware Decoupling

Virtual Try-On (VTON) aims to synthesize garment transfer without physical trials. Although recent methods perform well on upper-body garments, they still struggle in lower-body and full-body scenarios with complex occlusions and large silhouette changes. To address this limitation, we introduce ToWo (Take-Off Wear-On), a two-stage paradigm that decouples body structure estimation from garment synthesis. Take-Off first generates a tight-fitting body proxy that provides estimated structural guidance, and Wear-On then synthesizes the target garment conditioned on this prior. This decoupling reduces source-garment interference, supporting garment placement under substantial silhouette variations. Built on this paradigm, we propose ToWo-VTON, a unified topology-aware framework with structure-aware supervision. We construct the Body-Fitting DressCode (BFDC) dataset via body-aware diffusion and VLM-based filtering to provide body-proxy supervision across upper-, lower-, and full-body cases. We instantiate ToWo-VTON on both diffusion-based and MLLM-guided backbones. For diffusion-based models, we fine-tune on BFDC using the body proxy as the person input. For the MLLM-guided model, we use native backbone conditioning for the body proxy and target garment, and add Garment Boosting Attention (GBA) to preserve garment details. Experiments on VITON-HD and DressCode demonstrate improvements over the evaluated baselines, with KID reductions of 26.1% and 58.6% for diffusion-based and MLLM-guided implementations, respectively. The combined BFDC-training and Take-Off/Wear-On strategy also produces more coherent limb layouts and garment boundaries across the evaluated garment categories.

==> sec/3_pre.tex <==
\begin{comment}
\end{comment}

\section{Preliminaries}
\subsection{Multimodal Large Language Models}

\noindent\textbf{Autoregressive (AR) Encoding.}
The AR transformer autoregressively predicts interleaved multimodal tokens \cite{radford2018improving}. Given a sequence of tokens $s_{1:L}$, the generation probability is defined as:
\begin{equation}
p(s_{1:L}) = \prod_{\ell=1}^{L} p_\phi(s_\ell \mid s_{<\ell}),
\label{eq:arm}
\end{equation}
where $\phi$ denotes transformer parameters. The resulting hidden representation $h$ captures global multimodal context and serves as conditioning input for the diffusion stage.

\noindent\textbf{Latent Diffusion.}
A pretrained variational autoencoder (VAE) \cite{kingma2022autoencodingvariationalbayes} encodes the image into a latent vector $z_0 \!\in\! \mathbb{R}^d$, with the forward process:
\begin{equation}
q(z_t \mid z_0) = \mathcal{N}(z_t; \sqrt{\bar{\alpha}_t}z_0, (1-\bar{\alpha}_t)\mathbf{I}),
\label{eq:ldm}
\end{equation}
where $\bar{\alpha}_t = \prod_{s=1}^t \alpha_s$ and $\alpha_t = 1 - \beta_t$. The AR hidden state $h$ and latent feature $v = E(x)$ are refined individually to improve cross-modal alignment, then concatenated as $c = \mathrm{concat}(h', v')$. The diffusion model is trained via a velocity-matching objective \cite{liu2022flowstraightfastlearning}:
\begin{equation}
\mathcal{L}_{\mathrm{VM}} = \mathbb{E}_{z_t, t, c} \| v_\theta(z_t, t, c) - u_t(z_t) \|_2^2.
\label{eq:vmloss}
\end{equation}
%A multimodal rotary position embedding (M-RoPE) projects all tokens into a unified embedding space, promoting precise alignment between garment semantics and human structure for identity-preserving synthesis.


==> sec/LLM-usage.tex <==
\section*{LLM Usage Statement}

We used ChatGPT for manuscript drafting, revision and consistency checks. Research uses of generative models, including BooW-VTON/BSR, Qwen2.5-VL, and OmniGen2, are described in Section~3. GPT-5 and FLUX.1-Fill were used for background-prompt generation and background synthesis, respectively, as detailed in Appendix~C. The authors take responsibility for all content and results.

==> sec/statements.tex <==
\subsection*{AI use statement}

For manuscript preparation, we used generative AI tools only
for language polishing, including grammar correction and
improvements to clarity and readability.
We did not use AI assistance for research ideation, methodology
or experimental design, code development, or interpretation
of results.
As described in the paper, our research pipeline uses generative
models to construct body-fitting proxy images for $\mathcal{D}_{\text{BFDC}}$ and
vision-language models for proxy filtering and failure detection.
We reviewed all AI-assisted textual revisions to ensure that
they preserved the intended technical meaning.
We take full responsibility for the final content of this work,
including its text, claims, results, and artifacts.

\subsection*{Reproducibility statement}

To facilitate reproducibility, we describe the two-stage ToWo
framework and the construction and filtering procedures of $\mathcal{D}_{\text{BFDC}}$
in the main text.
Implementation details are provided in
Section~\ref{sec:implementation_detail}, including model
initialization, training datasets, Wear-On backbone configurations,
optimization settings, and computational hardware.


